Narcissus: Deriving Correct-By-Construction Decoders and Encoders from Binary Formats

It is a neat result from functional programming that libraries of parser combinators can support rapid construction of decoders for quite a range of formats. With a little more work, the same combinator program can denote both a decoder and an encoder. Unfortunately, the real world is full of gnarly formats, as with the packet formats that make up the standard Internet protocol stack. Most past parser-combinator approaches cannot handle these formats, and the few exceptions require redundancy -- one part of the natural grammar needs to be hand-translated into hints in multiple parts of a parser program. We show how to recover very natural and nonredundant format specifications, covering all popular network packet formats and generating both decoders and encoders automatically. The catch is that we use the Coq proof assistant to derive both kinds of artifacts using tactics, automatically, in a way that guarantees that they form inverses of each other. We used our approach to reimplement packet processing for a full Internet protocol stack, inserting our replacement into the OCaml-based MirageOS unikernel, resulting in minimal performance degradation.

==> Makefile <==
COMPATIBILITY_FILE=src/Common/Coq__8_4__8_5__Compat.v
STDTIME?=/usr/bin/time -f "$* (real: %e, user: %U, sys: %S, mem: %M ko)"

.PHONY: fiat fiat-core querystructures parsers parsers-examples parsers-examples-verbose parsers-all finitesets dns compiler facade-test ics fiat4monitors examples narcissus \
	fiat-quick fiat-core-quick querystructures-quick parsers-quick parsers-examples-quick parsers-examples-verbose-quick parsers-all-quick finitesets-quick dns-quick compiler-quick facade-test-quick ics-quick fiat4monitors-quick examples-quick narcissus-quick \
	install install-fiat install-fiat-core install-querystructures install-parsers install-parsers-examples install-parsers-examples-verbose install-parsers-all install-finitesets install-dns install-compiler install-ics install-fiat4monitors install-examples install-narcissus \
	pdf doc clean-doc \
	test-parsers test-parsers-profile test-parsers-profile-graph

ifneq (,$(wildcard .git)) # if we're in a git repo

# if the submodule changed, update it
SUBMODULE_DIFF=$(shell git diff etc/coq-scripts 2>&1 | grep 'Subproject commit')
SUBMODULE_DIRTY=$(shell git diff etc/coq-scripts 2>&1 | grep dirty)
ifneq (,$(SUBMODULE_DIRTY))
submodule-update::
	@ echo "\033[0;31mThe submodule is dirty; some scripts may fail.\033[0m"
	@ echo "\033[0;31mRun (cd etc/coq-scripts && git clean -xfd && git reset --hard)\033[0m"
else
ifneq (,$(SUBMODULE_DIFF))
submodule-update::
	git submodule sync && \
	git submodule update --init && \
	touch "$@"
endif
endif

ifeq (,$(wildcard submodule-update))
submodule-update::
	git submodule sync && \
	git submodule update --init && \
	touch "$@"
else
submodule-update::
endif

etc/coq-scripts/Makefile.coq.common etc/coq-scripts/compatibility/Makefile.coq.compat_84_85 etc/coq-scripts/compatibility/Makefile.coq.compat_84_85-early: submodule-update
	@ touch "$@"
endif

FAST_TARGETS += clean-doc etc/coq-scripts etc/coq-scripts/Makefile.coq.common etc/coq-scripts/compatibility/Makefile.coq.compat_84_85 etc/coq-scripts/compatibility/Makefile.coq.compat_84_85-early submodule-update
SUPER_FAST_TARGETS += submodule-update

Makefile.coq: etc/coq-scripts/Makefile.coq.common etc/coq-scripts/compatibility/Makefile.coq.compat_84_85 etc/coq-scripts/compatibility/Makefile.coq.compat_84_85-early

STRICT_COQDEP ?= 1

UPDATE_COQPROJECT = yes # always update _CoqProject, since we sometimes switch between ml4 and mlg
EXTRA_PIPE_SED_FOR_COQPROJECT = | sed s'/\.@ML4_OR_MLG@/.$(ML4_OR_MLG)/g'

include etc/coq-scripts/compatibility/Makefile.coq.compat_84_85-early

ifneq (,$(filter 8.4%,$(COQ_VERSION))) # 8.4 - this is a kludge to get around the fact that reinstalling 8.4 doesn't remove the 8.5 files, like universes.cmo
EXPECTED_EXT:=.v84
ML_DESCRIPTION := "Coq v8.4"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.5%,$(COQ_VERSION)))
EXPECTED_EXT:=.v85
ML_DESCRIPTION := "Coq v8.5"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.6%,$(COQ_VERSION)))
EXPECTED_EXT:=.v86
ML_DESCRIPTION := "Coq v8.6"
OTHERFLAGS += -w "-deprecated-appcontext -notation-overridden"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.7%,$(COQ_VERSION)))
EXPECTED_EXT:=.v87
ML_DESCRIPTION := "Coq v8.7"
OTHERFLAGS += -w "-deprecated-appcontext -notation-overridden"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.8%,$(COQ_VERSION)))
EXPECTED_EXT:=.v88
ML_DESCRIPTION := "Coq v8.8"
OTHERFLAGS += -w "-deprecated-appcontext -notation-overridden"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.9%,$(COQ_VERSION)))
EXPECTED_EXT:=.v89
ML_DESCRIPTION := "Coq v8.9"
OTHERFLAGS += -w "-deprecated-appcontext -notation-overridden"
ML4_OR_MLG := ml4
else
ifneq (,$(filter 8.10%,$(COQ_VERSION)))
EXPECTED_EXT:=.v810
ML_DESCRIPTION := "Coq v8.10"
OTHERFLAGS += -w "-deprecated-appcontext -notation-overridden"
ML4_OR_MLG := mlg
else
# >= 8.5 if it exists
NOT_EXISTS_LOC_DUMMY_LOC := $(call test_exists_ml_function,Loc.dummy_loc)

ifeq ($(NOT_EXISTS_LOC_DUMMY_LOC),1) # <= 8.4
EXPECTED_EXT:=.v84
ML_DESCRIPTION := "Coq v8.4"
ML4_OR_MLG := ml4
else
ifdef COQ_VERSION # if not, we're just going to remake the relevant Makefile to include anyway, so we shouldn't error
$(error Unrecognized Coq version $(COQ_VERSION))
endif
endif
endif
endif
endif
endif
endif
endif
endif

ML_COMPATIBILITY_FILES_PATTERN := src/Common/Tactics/hint_db_extra_tactics.ml src/Common/Tactics/hint_db_extra_plugin.@ML4_OR_MLG@ src/Common/Tactics/transparent_abstract_plugin.@ML4_OR_MLG@ src/Common/Tactics/transparent_abstract_tactics.ml

ML_COMPATIBILITY_FILES := $(subst @ML4_OR_MLG@,$(ML4_OR_MLG),$(ML_COMPATIBILITY_FILES_PATTERN))

include etc/coq-scripts/Makefile.coq.common

include etc/coq-scripts/compatibility/Makefile.coq.compat_84_85

ifeq ($(filter printdeps printreversedeps,$(MAKECMDGOALS)),)
-include etc/coq-scripts/Makefile.vo_closure
else
include etc/coq-scripts/Makefile.vo_closure
endif

.DEFAULT_GOAL := fiat

clean::
	rm -f src/Examples/Ics/WaterTank.ml
	rm -f submodule-update

clean-doc::
	rm -rf html
	rm -f all.pdf coqdoc.sty

HASNATDYNLINK = true

test-parsers: src/Parsers/Refinement/ExtractSharpenedABStar.vo
	$(MAKE) -C src/Parsers/Refinement/Testing

test-parsers-profile: src/Parsers/Refinement/ExtractSharpenedABStar.vo
	$(MAKE) -C src/Parsers/Refinement/Testing test-ab-star-profile

test-parsers-profile-graph: src/Parsers/Refinement/ExtractSharpenedABStar.vo
	$(MAKE) -C src/Parsers/Refinement/Testing test-ab-star-profile-graph

CORE_UNMADE_VO := \
	src/Common/ilist2.vo \
	src/Common/i2list.vo \
	src/Common/ilist2_pair.vo \
	src/Common/FMapExtensions/LiftRelationInstances.vo \
	src/Common/FMapExtensions/Wf.vo

QUERYSTRUCTURES_UNMADE_VO := \
	src/QueryStructure/Implementation/DataStructures/Bags/IndexedBags.vo \
	src/QueryStructure/Implementation/DataStructures/Bags/ProductBags.vo \
	src/QueryStructure/Implementation/DataStructures/Bags/InvertedIndexBags.vo

PARSERS_EXAMPLES_VERBOSE_UNMADE_VO := \
	src/Parsers/Refinement/SharpenedJavaScriptAssignmentExpression.vo

PARSERS_EXAMPLES_UNMADE_VO := \
	src/Parsers/Refinement/ExtractSharpenedJSComment.vo \
	src/Parsers/Refinement/ExtractSharpenedJSON.vo \
	$(PARSERS_EXAMPLES_VERBOSE_UNMADE_VO)

PARSERS_UNMADE_VO := \
	src/Parsers/Grammars/SimpleRecognizerOptimized.vo \
	src/Parsers/Refinement/SharpenedJSON.vo \
	$(PARSERS_EXAMPLES_UNMADE_VO)

FIAT4MONITORS_UNMADE_VO := \
	src/Fiat4Monitors/HelloWorld/%.vo \
	src/Fiat4Monitors/HealthMonitor/%.vo \
	src/Fiat4Monitors/TurretMonitorSpec.vo \
	src/Fiat4Monitors/MonitorRepInv.vo

EXAMPLES_UNMADE_VO := \
	src/Examples/Smtp/Smtp.vo \
	src/Examples/CacheADT/TrivialADTCache.vo \
	src/Examples/CacheADT/LRUCache.vo \
	src/Examples/CacheADT/KVEnsembles.vo \
	src/Examples/CacheADT/FMapCacheImplementation.vo \
	src/Examples/CacheADT/CacheSpec.vo \
	src/Examples/CacheADT/CacheSig.vo \
	src/Examples/CacheADT/CacheRefinements.vo \
	src/Examples/CacheADT/CacheADT.vo \
	src/Examples/QueryStructure/FriendFinder.vo \
	src/Examples/QueryStructure/Github.vo \
	src/Examples/QueryStructure/IncompleteROSMaster.vo \
	src/Examples/QueryStructure/Photoalbum.vo \
	src/Examples/QueryStructure/PhotoalbumExtraction.vo \
	src/Examples/QueryStructure/PhotoalbumUnOpt.vo \
	src/Examples/QueryStructure/PhotoalbumUnOptimizedExtraction.vo \
	src/Examples/QueryStructure/ProcessScheduler.vo \
	src/Examples/QueryStructure/DelegatedProcessScheduler.vo \
	src/Examples/QueryStructure/CodeLookup.vo \
	src/Examples/QueryStructure/SearchTest.vo \
	src/Examples/SearchTest.vo \
	src/Examples/Ics/WaterTankExtract.vo \
	src/Examples/HACMSDemo/WheelSensor.vo \
	src/Examples/HACMSDemo/WheelSensorEncoder.vo \
	src/Examples/HACMSDemo/WheelSensorDecoder.vo \
	src/Examples/HACMSDemo/WheelSensorExtraction.vo

EXTRACTION_UNMADE_VO := \
	src/CertifiedExtraction/Benchmarks/DNS.vo \

NARCISSUS_EXAMPLES_VO := \
	src/Narcissus/Examples/ByteAlignedExample.vo \
	src/Narcissus/Examples/ICMP_Packet.vo \
	src/Narcissus/Examples/IntExample.vo \
	src/Narcissus/Examples/NetworkStack/ARPPacket.vo \
	src/Narcissus/Examples/NetworkStack/EthernetFrame.vo \
	src/Narcissus/Examples/NetworkStack/EthernetHeader.vo \
	src/Narcissus/Examples/NetworkStack/Fiat4Mirage.vo \
	src/Narcissus/Examples/NetworkStack/TCP_Packet.vo \
	src/Narcissus/Examples/NetworkStack/UDP_Packet.vo \
	src/Narcissus/Examples/NetworkStack/IPv4Header.vo \
	src/Narcissus/Examples/DNS/DNSPacket.vo \
	src/Narcissus/Examples/DNS/DnsOpt.vo \
	src/Narcissus/Examples/DNS/RRecordTypes.vo \
	src/Narcissus/Examples/DNS/SimpleDNSPacket.vo \
	src/Narcissus/Examples/DNS/SimpleDnsOpt.vo \
	src/Narcissus/Examples/DNS/SimpleRRecordTypes.vo

NARCISSUS_UNMADE_VO := \
	src/Narcissus/Examples/Toy.vo \
	src/Narcissus/Examples/Toy2.vo \
	src/Narcissus/Formats/CInt.vo \
	src/Narcissus/BinLib/CharString.vo \
	src/Narcissus/Formats/ASN1.vo \
	$(NARCISSUS_EXAMPLES_VO)

WATER_TANK_EXTRACT_VO := src/Examples/Ics/WaterTankExtract.vo
WATER_TANK_EXTRACT_ML := src/Examples/Ics/WaterTank.ml

FIAT_CORE_VO := $(filter-out $(CORE_UNMADE_VO),$(filter src/Computation.vo src/ADT.vo src/ADTInduction.vo src/ADTNotation.vo src/ADTRefinement.vo src/Common.vo src/Computation/%.vo src/ADT/%.vo src/ADTNotation/%.vo src/ADTRefinement/%.vo src/Common/%.vo,$(VOFILES)))
QUERYSTRUCTURES_VO := $(filter-out $(QUERYSTRUCTURES_UNMADE_VO),$(filter src/QueryStructure/%.vo,$(VOFILES)))
PARSERS_VO := $(filter-out $(PARSERS_UNMADE_VO),$(filter src/Parsers/%.vo,$(VOFILES)))
PARSERS_EXAMPLES_VO := $(filter-out $(PARSERS_EXAMPLES_UNMADE_VO),$(filter src/Parsers/Refinement/Sharpened%.vo,$(VOFILES)))
PARSERS_EXAMPLES_VERBOSE_VO := $(filter-out $(PARSERS_EXAMPLES_VERBOSE_UNMADE_VO),$(filter src/Parsers/Refinement/ExtractSharpened%.vo,$(VOFILES)))
PARSERS_ALL_VO := $(filter src/Parsers/%.vo,$(VOFILES))
FINITESET_VO := $(filter src/FiniteSetADTs.vo src/FiniteSetADTs/%.vo,$(VOFILES))
DNS_VO := $(filter src/Examples/DnsServer/%.vo,$(VOFILES))
EXTRACTION_VO := $(filter-out $(EXTRACTION_UNMADE_VO),$(filter src/CertifiedExtraction/%.vo,$(VOFILES))) src/Examples/QueryStructure/ProcessScheduler.vo
FACADE_TEST_VO := src/Examples/FacadeTest.vo
ICS_VO := $(filter-out $(WATER_TANK_EXTRACT_VO),$(filter src/Examples/Ics/%.vo,$(VOFILES)))
TUTORIAL_VO := src/Examples/Tutorial/Tutorial.vo src/Examples/Tutorial/NotInList.vo src/Examples/Tutorial/Queue.vo src/Examples/Tutorial/BookstoreMoreManual.vo
HACMSDEMO_VO := src/Examples/HACMSDemo/DuplicateFree.vo src/Examples/HACMSDemo/HACMSDemo.vo src/Examples/HACMSDemo/WheelSensor.vo src/Examples/HACMSDemo/WheelSensorEncoder.vo src/Examples/HACMSDemo/WheelSensorDecoder.vo src/Examples/HACMSDemo/WheelSensorExtraction.vo
FIAT4MONITORS_VO := $(filter-out $(FIAT4MONITORS_UNMADE_VO), $(filter src/Fiat4Monitors/%.vo,$(VOFILES)))
EXAMPLES_VO := $(filter-out $(EXAMPLES_UNMADE_VO) $(ICS_VO) $(TUTORIAL_VO) $(DNS_VO) $(FACADE_TEST_VO),$(filter src/Examples/%.vo,$(VOFILES)))
NARCISSUS_VO := $(filter-out $(NARCISSUS_UNMADE_VO), $(filter src/Narcissus/%.vo,$(VOFILES)))
BEDROCK_VO := Bedrock/Nomega.vo Bedrock/Memory.vo Bedrock/Word.vo

FIAT_VO := $(FIAT_CORE_VO) $(QUERYSTRUCTURES_VO) $(PARSERS_VO)
TACTICS_TARGETS := $(filter src/Common/Tactics/%,$(CMOFILES) $(if $(HASNATDYNLINK_OR_EMPTY),$(CMXSFILES)))

fiat: $(FIAT_VO) $(TACTICS_TARGETS)
fiat-core: $(FIAT_CORE_VO) $(TACTICS_TARGETS)
querystructures: $(QUERYSTRUCTURES_VO)
parsers: $(PARSERS_VO)
parsers-examples: $(PARSERS_EXAMPLES_VO)
parsers-examples-verbose: $(PARSERS_EXAMPLES_VERBOSE_VO)
parsers-all: $(PARSERS_ALL_VO)
finitesets: $(FINITESETS_VO)
dns: $(DNS_VO)
extraction: $(EXTRACTION_VO)
facade-test: $(FACADE_TEST_VO)
ics: $(ICS_VO)
tutorial: $(TUTORIAL_VO)
hacms-demo: $(HACMSDEMO_VO)
fiat4monitors: $(FIAT4MONITORS_VO)
examples: $(EXAMPLES_VO)
bedrock: $(BEDROCK_VO)
narcissus: bedrock $(NARCISSUS_VO)
narcissus-examples: $(NARCISSUS_EXAMPLES_VO)

fiat-quick: $(addsuffix .vio,$(basename $(FIAT_VO))) $(TACTICS_TARGETS)
fiat-core-quick: $(addsuffix .vio,$(basename $(FIAT_CORE_VO))) $(TACTICS_TARGETS)
querystructures-quick: $(addsuffix .vio,$(basename $(QUERYSTRUCTURES_VO)))
parsers-quick: $(addsuffix .vio,$(basename $(PARSERS_VO)))
parsers-examples-quick: $(addsuffix .vio,$(basename $(PARSERS_EXAMPLES_VO)))
parsers-examples-verbose-quick: $(addsuffix .vio,$(basename $(PARSERS_EXAMPLES_VERBOSE_VO)))
parsers-all-quick: $(addsuffix .vio,$(basename $(PARSERS_ALL_VO)))
finitesets-quick: $(addsuffix .vio,$(basename $(FINITESETS_VO)))
dns-quick: $(addsuffix .vio,$(basename $(DNS_VO)))
facade-test-quick: $(addsuffix .vio,$(basename $(FACADE_TEST_VO)))
ics-quick: $(addsuffix .vio,$(basename $(ICS_VO)))
fiat4monitors-quick: $(addsuffix .vio,$(basename $(FIAT4MONITORS_VO)))
examples-quick: $(addsuffix .vio,$(basename $(EXAMPLES_VO)))
narcissus-quick: $(addsuffix .vio,$(basename $(NARCISSUS_VO)))

install-fiat: T = $(FIAT_VO)
install-fiat-core: T = $(FIAT_CORE_VO)
install-querystructures: T = $(QUERYSTRUCTURES_VO)
install-parsers: T = $(PARSERS_VO)
install-parsers-examples: T = $(PARSERS_EXAMPLES_VO)
install-parsers-examples-verbose: T = $(PARSERS_EXAMPLES_VERBOSE_VO)
install-parsers-all: T = $(PARSERS_ALL_VO)
install-finitesets: T = $(FINITESETS_VO)
install-dns: T = $(DNS_VO)
install-ics: T = $(ICS_VO)
install-fiat4monitors: T = $(FIAT4MONITORS_VO)
install-examples: T = $(EXAMPLES_VO)
install-narcissus: T = $(NARCISSUS_VO)

install-fiat install-fiat-core install-querystructures install-parsers install-parsers-examples install-parsers-examples-verbose install-parsers-all install-finitesets install-dns install-compiler install-fiat4monitors install-examples install-narcissus:
	$(SHOW)'MAKE -f Makefile.coq INSTALL'
	$(HIDE)$(MAKE) -f Makefile.coq VFILES="$(call vo_to_installv,$(T))" install

# This target is used to update the _CoqProject.in file.
# Use -R, not -I for Bedrock, as it is Coq input, not OCaml input.
$(UPDATE_COQPROJECT_TARGET):
	(echo '-R src Fiat'; echo '-R Bedrock Bedrock'; echo '-I src/Common/Tactics'; git ls-files "*.v" | grep -v '^$(COMPATIBILITY_FILE)$$' | $(SORT_COQPROJECT); (echo '$(COMPATIBILITY_FILE)'; git ls-files "*.{ml4,mlg}" | $(SORT_COQPROJECT); (echo '$(ML_COMPATIBILITY_FILES)' | tr ' ' '\n'; echo 'src/Common/Tactics/transparent_abstract_plugin.mllib'; echo 'src/Common/Tactics/hint_db_extra_plugin.mllib') | $(SORT_COQPROJECT))) > _CoqProject.in

ifeq ($(IS_FAST),0)
# see http://stackoverflow.com/a/9691619/377022 for why we need $(eval $(call ...))
$(eval $(call SET_ML_COMPATIBILITY,src/Common/Tactics/hint_db_extra_tactics.ml,$(EXPECTED_EXT)))
$(eval $(call SET_ML_COMPATIBILITY,src/Common/Tactics/hint_db_extra_plugin.$(ML4_OR_MLG),$(EXPECTED_EXT)))
$(eval $(call SET_ML_COMPATIBILITY,src/Common/Tactics/transparent_abstract_plugin.$(ML4_OR_MLG),$(EXPECTED_EXT)))
$(eval $(call SET_ML_COMPATIBILITY,src/Common/Tactics/transparent_abstract_tactics.ml,$(EXPECTED_EXT)))
endif


$(WATER_TANK_EXTRACT_ML): $(filter-out $(WATER_TANK_EXTRACT_VO),$(call vo_closure,$(WATER_TANK_EXTRACT_VO))) $(WATER_TANK_EXTRACT_VO:%.vo=%.v)
	$(SHOW)'COQC $(WATER_TANK_EXTRACT_VO:%.vo=%.v) > $@'
	$(HIDE)$(COQC) $(COQDEBUG) $(COQFLAGS) $(WATER_TANK_EXTRACT_VO:%.vo=%.v) > $@

src/Examples/QueryStructure/classifier.cmxa: src/Examples/QueryStructure/ClassifierExtraction.vo
	cd src/Examples/QueryStructure && ocamlopt -w -a -o classifier.cmxa -a classifier.mli classifier.ml

classifier_repl: src/Examples/QueryStructure/classifier_repl.ml src/Examples/QueryStructure/classifier.cmxa
	cd src/Examples/QueryStructure && ocamlopt -w -a -o classifier_repl unix.cmxa str.cmxa classifier.cmxa classifier_repl.ml

src/Examples/QueryStructure/classifier_unopt.cmxa: src/Examples/QueryStructure/ClassifierUnOptExtraction.vo
	cd src/Examples/QueryStructure && ocamlopt -w -a -o classifier_unopt.cmxa -a classifier_unopt.mli classifier_unopt.ml

classifierUnOpt_repl: src/Examples/QueryStructure/classifierUnOpt_repl.ml src/Examples/QueryStructure/classifier_unopt.cmxa
	cd src/Examples/QueryStructure && ocamlopt -w -a -o classifierUnOpt_repl unix.cmxa str.cmxa classifier_unopt.cmxa classifierUnOpt_repl.ml

src/Examples/HACMSDemo/wheelSensorEncoder.cmxa: src/examples/hacmsdemo/WheelSensorExtraction.vo
	cd src/Examples/HACMSDemo && ocamlopt -w -a -o wheelSensorEncoder.cmxa -a wheelSensorEncoder.mli wheelSensorEncoder.ml

encoder_repl: src/Examples/HACMSDemo/encoder_repl.ml src/Examples/HACMSDemo/wheelSensorEncoder.cmxa
	cd src/Examples/HACMSDemo && ocamlopt -w -a -o encoder_repl unix.cmxa str.cmxa wheelSensorEncoder.cmxa encoder_repl.ml

printdeps::
	$(HIDE)$(foreach vo,$(filter %.vo,$(MAKECMDGOALS)),echo '$(vo): $(call vo_closure,$(vo))'; )

printreversedeps::
	$(HIDE)$(foreach vo,$(filter %.vo,$(MAKECMDGOALS)),echo '$(vo): $(call vo_reverse_closure,$(VOFILES),$(vo))'; )


==> esh-preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT MODIFY THIS FILE %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Instead, redefine the relevant macros in your own source file, **after**
%% including this file.  This file is overwritten every time you run esh2tex
%% with the --write-preamble option.

%%%%%%%%%%%%%%
%% Core ESH %%
%%%%%%%%%%%%%%

\newcommand*{\ESHRequirePackage}[2][]
  {\IfFileExists{#2.sty}
    {\RequirePackage[#1]{#2}}
    {\PackageError{ESH}{Missing LaTeX dependency: please install #2}
      {ESH requires relsize, ulem, and xcolor to work properly.  On Debian derivatives, these packages are provided by texlive-recommended and texlive-latex-extra.}}}

% Packages
%%%%%%%%%%

\ESHRequirePackage{xcolor} % TeXLive-recommended
\ESHRequirePackage[normalem]{ulem} % TeXLive-recommended

\ESHRequirePackage{relsize} % TeXLive-latex-extra
\renewcommand{\RSsmallest}{1pt}
\renewcommand{\RSlargest}{50pt}

% Fonts
%%%%%%%

% Code blocks
\newcommand*{\ESHFontSize}{}
\newcommand*{\ESHFontFamily}{\ttfamily}
\newcommand*{\ESHFont}{\ESHFontSize\ESHFontFamily}

% Inline snippets
\newcommand*{\ESHInlineFontSize}{\ESHFontSize}
\newcommand*{\ESHInlineFontFamily}{\ESHFontFamily}
\newcommand*{\ESHInlineFont}{\ESHInlineFontSize\ESHInlineFontFamily}

% Inline blocks
\newcommand*{\ESHInlineBlockFontSize}{\ESHFontSize}
\newcommand*{\ESHInlineBlockFontFamily}{\ESHFontFamily}
\newcommand*{\ESHInlineBlockFont}{\ESHInlineBlockFontSize\ESHInlineBlockFontFamily}

% Blocks
\newcommand*{\ESHBlockFontSize}{\ESHFontSize}
\newcommand*{\ESHBlockFontFamily}{\ESHFontFamily}
\newcommand*{\ESHBlockFont}{\ESHBlockFontSize\ESHBlockFontFamily}

% Characters not covered by \ESHFont (XeTeX/LuaTeX only)
\newcommand*{\ESHFallbackFontFamily}{\ESHFontFamily}
\newcommand*{\ESHFallbackFont}{\ESHFallbackFontFamily}

% Utils
%%%%%%%

% \ESHNoHyphens disables hyphenation
\newcommand*{\ESHNoHyphens}{\hyphenpenalty=10000}

% \ESHConstantSpace ensures that spaces can't stretch
\newcommand*{\ESHConstantSpace}{\spaceskip=\fontdimen2\font\xspaceskip=0pt}

% \ESHCenterInWidthOf{#A}{#B} prints #B centered in a box as large as #A.
\newdimen\ESHtempdim%
\newcommand*{\ESHCenterInWidthOf}[2]
  {\settowidth\ESHtempdim{#1}%
   \makebox[\ESHtempdim][c]{#2}}

% ESHText switches out of math mode if needed (textnormal amstext-friendly)
\DeclareRobustCommand*{\ESHText}[1]{\ifmmode{\textnormal{#1}}\else{#1}\fi}

% \ESHIfFontChar{#A} uses a XeLaTeX/LuaTeX primitive to print #A in
% \ESHFallbackFont if it isn't covered by the current font.
\newcommand*{\ESHIfFontChar}[1]
  {\iffontchar\font`#1{#1}\else{\ESHFallbackFont#1}\fi}

\makeatletter
% In XeTeX and LuaTeX, \ESHWithFallback{#A} prints #A in the current font if
% possible and falls back to \ESHFallbackFont. In other engines, it always uses
% the fallback font.  The XeTeX implementation is derived from
% https://tug.org/pipermail/xetex/2011-November/022319.html.
\@ifundefined{XeTeXinterchartoks}
  {\@ifundefined{luatexversion}
     {% Not using XeTeX, nor LuaTeX: fall back to just using \ESHFallbackFont
      \def\ESHWithFallback#1{\ESHFallbackFont#1}}
     {% Using LuaTeX
      \def\ESHWithFallback#1{\ESHIfFontChar{#1}}}}
  {% Using XeTeX
   \def\ESHWithFallback#1{%
     \ifnum\XeTeXfonttype\font>0% Graphite, OpenType, or AAT font
       \ESHIfFontChar{#1}%
     \else% Legacy TeX font
       \setbox0=\hbox{\tracinglostchars=0\kern1sp#1\expandafter}%
       \ifnum\lastkern=1{\ESHFallbackFont#1}\else{#1}\fi
     \fi}}
\makeatother

% \ESH*SpecialChar is used to wrap non-ascii characters, which may need a fallback font
\DeclareRobustCommand*{\ESHInlineSpecialChar}[1]
  {{\ESHInlineFontFamily\ESHWithFallback{#1}}}
\DeclareRobustCommand*{\ESHBlockSpecialChar}[1]
  {{\ESHCenterInWidthOf{\ESHBlockFontFamily{a}}{\ESHBlockFontFamily\ESHWithFallback{#1}}}}
% \ESH*UnicodeSubstitution is for special characters replaced by equivalent math commands
\DeclareRobustCommand*{\ESHInlineUnicodeSubstitution}[1]
  {{\ESHInlineFontFamily#1}}
\DeclareRobustCommand*{\ESHBlockUnicodeSubstitution}[1]
  {{\ESHCenterInWidthOf{\ESHBlockFontFamily{a}}{\ESHBlockFontFamily#1}}}
\DeclareRobustCommand*{\ESHMathSymbol}[1]{\ensuremath{#1}}

% \ESHSetCurFontSize sets \ESHCurFontSize to the current font size (1 CSS em)
\makeatletter
\newlength{\ESHCurFontSize}
\newcommand*{\ESHSetCurFontSize}{\setlength{\ESHCurFontSize}{\f@size pt}}
\makeatother

% \ESH*Raise implements sub/superscripts
\DeclareRobustCommand*{\ESHInlineRaise}[2]
  {\ESHSetCurFontSize\raisebox{#1\ESHCurFontSize}{\relsize{-2}#2}}
\DeclareRobustCommand*{\ESHBlockRaise}[2]
  {\rlap{\ESHInlineRaise{#1}{#2}}\hphantom{#2}}

% ESH*Strut implements struts
\newlength{\ESHBaselineskip}
\DeclareRobustCommand*{\ESHBlockStrut}[1]
  {\rule{0pt}{#1\ESHBaselineskip}}

\makeatletter
% ESHUnderline produces a straight underline
\DeclareRobustCommand*{\ESHUnderline}[1]
  {\bgroup\UL@setULdepth\markoverwith{#1\rule[-\ULdepth]{2pt}{0.4pt}}\ULon}
% ESHUnderwave produces a wavy underline
\DeclareRobustCommand*{\ESHUnderwave}[1]
  {\bgroup\UL@setULdepth\markoverwith{#1\raisebox{-\ULdepth}{\raisebox{-.5\height}{\ESHSmallWaveFont\char58}}}\ULon}
\font\ESHSmallWaveFont=lasyb10 scaled 400
\makeatother

% \ESHBoxSep is the vertical padding of \ESHBox
\newlength{\ESHBoxSep}
\setlength{\ESHBoxSep}{1pt}

% \ESHPhantomStrut{} adds a zero-width strut whose depth and height are that of "Ag"
\newcommand*{\ESHPhantomStrut}{\vphantom{Ag}}

% \ESHBox{#color}{#lineWidth}{#contents} wraps #contents in an border of width
% #lineWidth and of color #color.  The box has no horizontal padding, its
% vertical padding is determined by \ESHBoxSep, and it doesn't affect the height
% of the current line.
\newdimen\ESHBoxTempDim%
\newcommand*{\ESHBox}[3]
  {\setlength{\fboxsep}{\ESHBoxSep}%
   \setlength{\fboxrule}{#2}%
   \setlength{\ESHBoxTempDim}{\dimexpr-\fboxsep-\fboxrule\relax}%
   \ESHPhantomStrut{}\vphantom{#3}%
   \smash{\fbox{\hspace*{\ESHBoxTempDim}\ESHPhantomStrut{}#3\hspace*{\ESHBoxTempDim}}}}

% \ESHColorBox{#color}{#contents} adds a background of color #color to
% #contents.  The box has no horizontal padding, its vertical padding is
% determined by \ESHBoxSep, and it doesn't affect the height of the current
% line.
\newcommand*{\ESHColorBox}[2]
  {\setlength{\fboxsep}{\ESHBoxSep}%
   \setlength{\ESHBoxTempDim}{\dimexpr-\fboxsep-\fboxrule\relax}%
   \ESHPhantomStrut{}\vphantom{#2}%
   \smash{\colorbox[HTML]{#1}{\hspace*{\ESHBoxTempDim}\ESHPhantomStrut{}#2\hspace*{\ESHBoxTempDim}}}}

% \ESHWeight* and \ESH*Slant* adjust weight and slant
\newcommand*{\ESHWeightLight}[1]{\textlf{#1}}
\newcommand*{\ESHWeightRegular}[1]{\textmd{#1}}
\newcommand*{\ESHWeightBold}[1]{\textbf{#1}}
\newcommand*{\ESHInlineSlantItalic}[1]{\textit{#1}}
\newcommand*{\ESHBlockSlantItalic}[1]{{\itshape{#1}}} % No italic correction
\newcommand*{\ESHInlineSlantOblique}[1]{\textsl{#1}}
\newcommand*{\ESHBlockSlantOblique}[1]{{\slshape{#1}}}
\newcommand*{\ESHSlantNormal}[1]{\textup{#1}}

% Environments and macros
%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\ESHBreakingSpace}{\ }
\newcommand*{\ESHNonbreakingSpace}{\nobreakspace}

% Internal plumbing needed to make the same code work with Inline, Block, and
% InlineBlock.  See http://tex.stackexchange.com/questions/336936/ for details.
\let\ESHSpecialChar\ignorespaces%
\let\ESHUnicodeSubstitution\ignorespaces%
\let\ESHRaise\ignorespaces%
\let\ESHBol\ignorespaces%
% ESH*EmptyLine is inserted on every empty line of code to prevent LaTeX from
% complaining about underfull boxes
\let\ESHEmptyLine\ignorespaces%
\let\ESHEol\ignorespaces%
\let\ESHSpace\ignorespaces%
\let\ESHDash\ignorespaces%
\let\ESHSlantItalic\ignorespaces%
\DeclareRobustCommand*{\ESHInlineInternalSetup}
  {\def\ESHSpecialChar{\ESHInlineSpecialChar}\def\ESHUnicodeSubstitution{\ESHInlineUnicodeSubstitution}%
   \def\ESHRaise{\ESHInlineRaise}\def\ESHSlantItalic{\ESHInlineSlantItalic}%
   \def\ESHStrut{\relax}\def\ESHBol{\relax}\def\ESHEmptyLine{\mbox{}}\def\ESHEol{\newline}%
   \def\ESHSpace{\ESHBreakingSpace}%
   \def\ESHDash{-}}
\DeclareRobustCommand*{\ESHInlineBlockInternalSetup}
  {\def\arraystretch{1}%
   \def\ESHSpecialChar{\ESHBlockSpecialChar}\def\ESHUnicodeSubstitution{\ESHBlockUnicodeSubstitution}%
   \def\ESHRaise{\ESHBlockRaise}\def\ESHSlantItalic{\ESHBlockSlantItalic}%
   \setlength{\ESHBaselineskip}{\baselineskip}\def\ESHStrut{\ESHBlockStrut}%
   \def\ESHBol{\-}\def\ESHEmptyLine{\mbox{}}\def\ESHEol{\cr}%
   \def\ESHSpace{\ESHNonbreakingSpace}\def\ESHDash{\hbox{-}\nobreak}}
\DeclareRobustCommand*{\ESHBlockInternalSetup}
  {\def\ESHSpecialChar{\ESHBlockSpecialChar}\def\ESHUnicodeSubstitution{\ESHBlockUnicodeSubstitution}%
   \def\ESHRaise{\ESHBlockRaise}\def\ESHSlantItalic{\ESHBlockSlantItalic}%
   \setlength{\ESHBaselineskip}{\baselineskip}\def\ESHStrut{\ESHBlockStrut}%
   \def\ESHBol{\-}\def\ESHEmptyLine{\mbox{}}\def\ESHEol{\newline}%
   \def\ESHSpace{\ESHNonbreakingSpace}\def\ESHDash{\hbox{-}\nobreak}}

% Basic setup used when entering each type of environment or macro
% See http://tex.stackexchange.com/questions/22852 for \leavevmode
% \ESHBlockBasicSetup used to set \parskip to 0, but \ESHEol isn't \par anymore
\newcommand*{\ESHInlineBasicSetup}
  {\leavevmode\ESHNoHyphens\ESHInlineFont}
\newcommand*{\ESHInlineBlockBasicSetup}
  {\ESHNoHyphens\ESHInlineBlockFont\ESHConstantSpace}
\newcommand*{\ESHBlockBasicSetup}
  {\setlength{\parindent}{0pt}\raggedright\ESHNoHyphens%
   \ESHBlockFont\ESHConstantSpace}

% ESH*Hook is used to inject code before every ESH segment
\newcommand*{\ESHHook}{}
\newcommand*{\ESHInlineHook}{\ESHHook}
\newcommand*{\ESHInlineBlockHook}{\ESHHook}
\newcommand*{\ESHBlockHook}{\ESHHook}

\makeatletter
% \ESHInline is used for inline code
\DeclareRobustCommand*{\ESHInline}[1]
  {\bgroup\ESHText{\ESHInlineInternalSetup\ESHInlineBasicSetup\ESHInlineHook#1}\egroup}

% \ESHInlineBlockVerticalAlignment is the default vertical alignment of inline blocks
\newcommand*{\ESHInlineBlockVerticalAlignment}{c}

% \ESHInlineBlock is used for inline code blocks
\newenvironment{ESHInlineBlock}[1][\ESHInlineBlockVerticalAlignment]
  {\bgroup\ESHInlineBlockInternalSetup\ESHInlineBlockBasicSetup\ESHInlineBlockHook\begin{tabular}[#1]{@{}l@{}}}
  {\end{tabular}\egroup}

% \ESHSkip is the amount to skip before and after an \ESHBlock
\newlength{\ESHSkip}
\setlength{\ESHSkip}{\baselineskip}

% \ESHNoBreakAddVSpace adds vertical space, but prevents a page break.
% \nobreak would use a \penalty (which breaks \addvspace), hence \addpenalty.
\newcommand*{\ESHNoBreakAddVSpace}[1]{\addpenalty{\@M}\addvspace{#1}}

% \ESHBlock is used for code blocks
\newenvironment{ESHBlock}
  {\par\ESHNoBreakAddVSpace{\ESHSkip}\bgroup\ESHBlockInternalSetup\ESHBlockBasicSetup\ESHBlockHook}
  {\par\egroup\addvspace{\ESHSkip}}
\makeatother

%% \input wrappers
%%%%%%%%%%%%%%%%%%

\DeclareRobustCommand*{\ESHInputInline}[1]{\ESHInline{\input{#1.esh.tex}\unskip}}
\DeclareRobustCommand*{\ESHInputInlineBlock}[2][\ESHInlineBlockVerticalAlignment]
  {\begin{ESHInlineBlock}[#1]\input{#2.esh.tex}\unskip\end{ESHInlineBlock}}
\DeclareRobustCommand*{\ESHInputBlock}[1]{\begin{ESHBlock}\input{#1.esh.tex}\unskip\end{ESHBlock}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \ESHpv: ESH Precomputed-Verbs support %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Adapted from https://tex.stackexchange.com/questions/336837/

%% Utilities

% \ESHpvEnterVerbMode sets all specials to catcode 12
% * \@makeother sets the catcode of its argument to 12 (other)
% * \dospecials applies \do to each special character
% (see http://tex.stackexchange.com/questions/12721/control-command-arguments)
\makeatletter
\def\ESHpvEnterVerbMode{\let\do\@makeother\dospecials}
\makeatother

% \ESHpvNotFound{#msg} issues a warning
\def\ESHpvNotFoundMessage#1{No highlighting found for "#1"; falling back to verbatim.}
\def\ESHpvNotFound#1{\PackageWarning{ESH}{\ESHpvNotFoundMessage{#1}}}

%% Defining substitutions

% ESHpvReadDelimitedAndDefineSubstitution{#lang}#delim#key#delim#value maps
% #lang-\detokenize{#key} to #value
\def\ESHpvReadDelimitedAndDefineSubstitution#1#2{%
  % \ESHpvInternalScanner reads tokens up to the next separator #2, restores
  % catcodes (\endgroup), and calls \ESHpvDefineSubstitution on these tokens
  \def\ESHpvInternalScanner##1#2{\endgroup\ESHpvDefineSubstitution{#1}{##1}}\ESHpvInternalScanner}

% ESHpvDefineSubstitution{#lang}{#key}#value maps #lang-\detokenize{#key} to #value
\def\ESHpvDefineSubstitution#1#2{\expandafter\def\csname #1-\detokenize{#2}\endcsname}

%% Applying substitutions

% \ESHpvSubstitute{#lang}{#key}{#msg}{#fallback} looks up a mapping for
% #lang-\detokenize{#key} and inserts it.  If no mapping can be found, it prints
% a warning based on #msg and includes #fallback in the document.
\def\ESHpvSubstitute#1#2#3#4{%
  \expandafter\ifx\csname #1-\detokenize{#2}\endcsname\relax
  \ESHpvNotFound{#3}\texttt{#4}%
  \else
  \csname #1-\detokenize{#2}\expandafter\endcsname
  \fi}

% \ESHpvSubstituteMacro{#lang}{#key} looks up #lang-\detokenize{#key} and
% substitutes it.  It falls back to #key itself if no mapping can be found.
\def\ESHpvSubstituteMacro#1#2{\ESHpvSubstitute{#1}{#2}{\detokenize{#2}}{\detokenize{#2}}}

% ESHpvReadDelimitedAndSubstitute{#lang}#delim#key#delim looks up
% #lang-\detokenize{#key} and calls \ESHpvSubstituteMacro.
\def\ESHpvReadDelimitedAndSubstitute#1#2{%
  % \ESHpvInternalScanner reads tokens up to the next separator #2, restores
  % catcodes (\endgroup), and calls \ESHpvSubstituteMacro on these tokens
  \def\ESHpvInternalScanner##1#2{\endgroup\ESHpvSubstituteMacro{#1}{##1}}\ESHpvInternalScanner}

%% High-level interface

% \ESHpvLookupVerb reads its argument like \verb
% Note that this won't work perfectly as an argument to a macro
\DeclareRobustCommand*{\ESHpvLookupVerb}[1]
  {\begingroup\ESHpvEnterVerbMode\ESHpvReadDelimitedAndSubstitute{macro-#1}}

% \ESHpvDefineVerb#lang creates a new [code → highlight] record in table macro-#A
\DeclareRobustCommand*{\ESHpvDefineVerb}[1]
  {\begingroup\ESHpvEnterVerbMode\ESHpvReadDelimitedAndDefineSubstitution{macro-#1}}

%% Convenience functions for wrapping verbs in boxes

\newcommand*{\ESHSaveBoxName}[1]{ESHSaveBox:#1}

\makeatletter
% \ESHEnsureSaveBox{#name} calls \newsavebox{#name} if needed.
\newcommand{\ESHEnsureSaveBox}[1]
  {\@ifundefined{#1}{\expandafter\newsavebox\csname#1\endcsname}{}}
\makeatother

% \begin{ESHSavedVerb}{#name}#def\end{ESHSavedVerb} creates a box called
% ESHSaveBox:#name, and saves #def into it.
\newenvironment*{ESHSavedVerb}[1]
  {\def\ESHCurBox{\ESHSaveBoxName{#1}}\ESHEnsureSaveBox{\ESHCurBox}\begin{lrbox}{0}\ignorespaces}
  {\unskip\end{lrbox}\global\expandafter\setbox\csname\ESHCurBox\endcsname=\box0\relax}

% \ESHUseVerb{#name} retrieves the contents of the box ESHSaveBox:#name
\newcommand{\ESHUseVerb}[1]{\expandafter\usebox\csname\ESHSaveBoxName{#1}\endcsname}


==> listings/constraints0cond.v.esh.tex <==
\ESHBol{}\{s\ESHSpace{}|\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}\}

==> listings/constraints0fmt.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationId\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\epsilon}}

==> listings/constraints1cond.v.esh.tex <==
\ESHBol{}\{s\ESHSpace{}|\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}s.stationId\ESHSpace{}=\ESHSpace{}w\}

==> listings/constraints1fmt.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\epsilon}}

==> listings/constraints2cond.v.esh.tex <==
\ESHBol{}\{s\ESHSpace{}|\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}s.stationId\ESHSpace{}=\ESHSpace{}w\}

==> listings/constraints2fmt.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\epsilon}}

==> listings/constraints3cond.v.esh.tex <==
\ESHBol{}\{s\ESHSpace{}|\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}s.stationId\ESHSpace{}=\ESHSpace{}w\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}=\ESHSpace{}ln\}

==> listings/constraints3fmt.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data

==> listings/constraints4cond.v.esh.tex <==
\ESHBol{}\{s\ESHSpace{}|\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}s.stationId\ESHSpace{}=\ESHSpace{}w\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}length\ESHSpace{}s.data\ESHSpace{}=\ESHSpace{}ln\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\wedge}}\ESHSpace{}s.data\ESHSpace{}=\ESHSpace{}l\}

==> listings/constraints4fmt.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\epsilon}}

==> listings/derivation0impl.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{s}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}t\ESHRaise{-0.25}{1}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}encode\_word\ESHSpace{}s.stationId;\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}t\ESHRaise{-0.25}{2}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\ESHUnicodeSubstitution{\scalebox{0.75}{\ensuremath{\square}}};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(t\ESHRaise{-0.25}{1}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}t\ESHRaise{-0.25}{2})

==> listings/derivation0spec.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationId\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data

==> listings/derivation1impl.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{s}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}t\ESHRaise{-0.25}{2}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}encode\_word\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00000000;\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}t\ESHRaise{-0.25}{3}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\ESHUnicodeSubstitution{\scalebox{0.75}{\ensuremath{\square}}};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(t\ESHRaise{-0.25}{2}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}t\ESHRaise{-0.25}{3})

==> listings/derivation1spec.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data

==> listings/derivation2impl.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{s}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}t\ESHRaise{-0.25}{3}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}encode\_nat\ESHSpace{}(length\ESHSpace{}s.data);\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}t\ESHRaise{-0.25}{4}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\ESHUnicodeSubstitution{\scalebox{0.75}{\ensuremath{\square}}};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(t\ESHRaise{-0.25}{3}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}t\ESHRaise{-0.25}{4})

==> listings/derivation2spec.v.esh.tex <==
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data

==> listings/derivation3impl.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{s}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(encode\_list\ESHSpace{}encode\_word\ESHSpace{}s.data)

==> listings/derivation3spec.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data

==> listings/ipchecksumtac.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Ltac}\ESHSpace{}\textcolor[HTML]{A40000}{apply\_new\_combinator\_rule}\ESHSpace{}::=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{204A87}{match}\ESHSpace{}goal\ESHSpace{}\textcolor[HTML]{204A87}{with}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}[\ESHSpace{}H\ESHSpace{}:\ESHSpace{}cache\_inv\_Property\ESHSpace{}\_\ESHSpace{}\_\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\vdash}}\ESHSpace{}CorrectDecoder\ESHSpace{}\_\ESHSpace{}\_\ESHSpace{}\_\ESHSpace{}\_\ESHSpace{}(\textcolor[HTML]{B35000}{?fmt\ESHRaise{-0.25}{1}}\ESHSpace{}\textcolor[HTML]{75507B}{ThenChecksum}\ESHSpace{}\_\ESHSpace{}\textcolor[HTML]{75507B}{OfSize}\ESHSpace{}\_\ESHSpace{}\textcolor[HTML]{75507B}{ThenCarryOn}\ESHSpace{}\textcolor[HTML]{B35000}{?fmt\ESHRaise{-0.25}{2}})\ESHSpace{}\_\ESHSpace{}\_\ESHSpace{}\_\ESHSpace{}]\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{00008B}{eapply}\ESHSpace{}compose\_IPChecksum\_format\_correct{'}\ESHSpace{}\textcolor[HTML]{204A87}{with}\ESHSpace{}(format\ESHRaise{-0.25}{1}\ESHSpace{}:=\ESHSpace{}fmt\ESHRaise{-0.25}{1});\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}[\ESHSpace{}\textcolor[HTML]{FF0000}{exact}\ESHSpace{}H\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}\textcolor[HTML]{B452CD}{repeat}\ESHSpace{}calculate\_length\_ByteString\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}\textcolor[HTML]{B452CD}{repeat}\ESHSpace{}calculate\_length\_ByteString\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}solve\_mod\_8\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}solve\_mod\_8\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}normalize\_format;\ESHSpace{}apply\_rules\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}normalize\_format;\ESHSpace{}apply\_rules\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}solve\_Prefix\_Format\ESHSpace{}]\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{204A87}{end}.

==> listings/ipv4fmt.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{IPv4\_format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}(\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}4\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}(constant\ESHSpace{}4)\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}4\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}(plus\ESHSpace{}5)\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{204A87}{@}}length\ESHSpace{}\_\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}Options\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHSpace{}\ESHSlantItalic{\textcolor[HTML]{5F615C}{(*\ESHSpace{}TOS\ESHSpace{}Field!\ESHSpace{}*)}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}TotalLength\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}ID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}1\ESHSpace{}\ESHSlantItalic{\textcolor[HTML]{5F615C}{(*\ESHSpace{}Unused\ESHSpace{}flag!\ESHSpace{}*)}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_bool}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}DF\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_bool}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}MF\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}FragmentOffset\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}TTL\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_enum}\ESHSpace{}ProtocolTypeCodes\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}Protocol)\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{ThenChecksum}\ESHSpace{}IPChecksum\_Valid\ESHSpace{}\textcolor[HTML]{75507B}{OfSize}\ESHSpace{}16\ESHSpace{}\textcolor[HTML]{75507B}{ThenCarryOn}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}(\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}SourceAddress\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}DestAddress\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}Options).

==> listings/sensor0dec.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{decode}\ESHSpace{}:=\ESHSpace{}decoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{0}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}w\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}b\ESHRaise{-0.25}{0}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}b{'};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}\{|\ESHSpace{}stationID\ESHSpace{}:=\ESHSpace{}b;\ESHSpace{}data\ESHSpace{}:=\ESHSpace{}w\ESHSpace{}|\}

==> listings/sensor0def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Record}\ESHSpace{}\textcolor[HTML]{A40000}{sensor\_msg}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\{\ESHSpace{}stationID:\ESHSpace{}word\ESHSpace{}8;\ESHSpace{}data:\ESHSpace{}word\ESHSpace{}16\ESHSpace{}\}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHSpace{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\top}}}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_dec}:\ESHSpace{}EncDecPair\ESHSpace{}format\ESHSpace{}invariant\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{75507B}{ltac}}:(\textcolor[HTML]{00008B}{derive\_encoder\_decoder\_pair}).

==> listings/sensor0enc.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{encode}\ESHSpace{}:=\ESHSpace{}encoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}stationID\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}data\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}(high\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}low\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte})

==> listings/sensor1dec.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{decode}\ESHSpace{}:=\ESHSpace{}decoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\_\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}w\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}b{'};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}\{|\ESHSpace{}stationID\ESHSpace{}:=\ESHSpace{}b;\ESHSpace{}data\ESHSpace{}:=\ESHSpace{}w\ESHSpace{}|\}

==> listings/sensor1def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Record}\ESHSpace{}\textcolor[HTML]{A40000}{sensor\_msg}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\{\ESHSpace{}stationID:\ESHSpace{}word\ESHSpace{}8;\ESHSpace{}data:\ESHSpace{}word\ESHSpace{}16\ESHSpace{}\}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHSpace{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\top}}}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_dec}:\ESHSpace{}EncDecPair\ESHSpace{}format\ESHSpace{}invariant\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{75507B}{ltac}}:(\textcolor[HTML]{00008B}{derive\_encoder\_decoder\_pair}).

==> listings/sensor1enc.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{encode}\ESHSpace{}:=\ESHSpace{}encoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}stationID\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00000000\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}data\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}(high\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}low\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte})

==> listings/sensor2dec.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{decode}\ESHSpace{}:=\ESHSpace{}decoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\_\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}w\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}b{'};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}(\textcolor[HTML]{204A87}{if}\ESHSpace{}weq\ESHSpace{}w\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}0000011111100010\ESHSpace{}\textcolor[HTML]{204A87}{then}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{2}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}b{'}\ESHRaise{-0.25}{0}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}w\ESHRaise{-0.25}{0}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}b\ESHRaise{-0.25}{2}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}b{'}\ESHRaise{-0.25}{0};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{204A87}{match}\ESHSpace{}index\ESHSpace{}(high\_bits\ESHSpace{}2\ESHSpace{}w\ESHRaise{-0.25}{0})\ESHSpace{}[0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00;\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}01]\ESHSpace{}\textcolor[HTML]{204A87}{with}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}Some\ESHSpace{}a{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\rightarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}\{|\ESHSpace{}stationID\ESHSpace{}:=\ESHSpace{}b;\ESHSpace{}data\ESHSpace{}:=\ESHSpace{}(a{'},\ESHSpace{}low\_bits\ESHSpace{}14\ESHSpace{}w\ESHRaise{-0.25}{0})\ESHSpace{}|\}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}None\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\rightarrow}}\ESHSpace{}\textcolor[HTML]{346604}{fail}\ESHSpace{}\textcolor[HTML]{204A87}{end}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{204A87}{else}\ESHSpace{}\textcolor[HTML]{346604}{fail})

==> listings/sensor2def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{kind}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}EnumType\ESHSpace{}[\textcolor[HTML]{5C3566}{"TEMP"};\ESHSpace{}\textcolor[HTML]{5C3566}{"HUMIDITY"}].\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Record}\ESHSpace{}\textcolor[HTML]{A40000}{sensor\_msg}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\{\ESHSpace{}stationID:\ESHSpace{}word\ESHSpace{}8;\ESHSpace{}data:\ESHSpace{}(kind\ESHSpace{}*\ESHSpace{}word\ESHSpace{}14)\ESHSpace{}\}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_const}\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}0000011111100010\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_enum}\ESHSpace{}[0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00;\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}01]\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}fst\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}snd\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHSpace{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\top}}}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_dec}:\ESHSpace{}EncDecPair\ESHSpace{}format\ESHSpace{}invariant\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{75507B}{ltac}}:(\textcolor[HTML]{00008B}{derive\_encoder\_decoder\_pair}).

==> listings/sensor2enc.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{encode}\ESHSpace{}:=\ESHSpace{}encoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}stationID\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00000000\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00000111\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}11100010\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}(\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{r}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}(Vector.nth\ESHSpace{}[0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00;\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}01]\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\circ}}\ESHSpace{}fst\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\circ}}\ESHSpace{}data)\ESHSpace{}r\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}(snd\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\circ}}\ESHSpace{}data)\ESHSpace{}r)\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}(high\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}low\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte})

==> listings/sensor3def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Record}\ESHSpace{}\textcolor[HTML]{A40000}{sensor\_msg}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\{\ESHSpace{}stationID:\ESHSpace{}word\ESHSpace{}8;\ESHSpace{}data:\ESHSpace{}list\ESHSpace{}(word\ESHSpace{}16)\ESHSpace{}\}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_unused\_word}\ESHSpace{}8\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_const}\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}0000011111100010\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHSpace{}\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\top}}}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_dec}:\ESHSpace{}EncDecPair\ESHSpace{}format\ESHSpace{}invariant\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{75507B}{ltac}}:(\textcolor[HTML]{00008B}{derive\_encoder\_decoder\_pair}).

==> listings/sensor4def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_const}\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}0000011111100010\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.

==> listings/sensor5dec.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{decode}\ESHSpace{}:=\ESHSpace{}decoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{0}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}b{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}w\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}b\ESHRaise{-0.25}{1}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}b{'};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}(\textcolor[HTML]{204A87}{if}\ESHSpace{}weq\ESHSpace{}w\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}0000011111100010\ESHSpace{}\textcolor[HTML]{204A87}{then}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}l\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}ListAlignedDecodeM\ESHSpace{}(\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{\_}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}w\ESHRaise{-0.25}{0}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}w{'}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\leftarrow}}\ESHSpace{}\textcolor[HTML]{75507B}{GetCurrentByte};\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}w\ESHRaise{-0.25}{0}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}w{'})\ESHSpace{}(wordToNat\ESHSpace{}b\ESHRaise{-0.25}{0});\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}\{|\ESHSpace{}stationID\ESHSpace{}:=\ESHSpace{}b;\ESHSpace{}data\ESHSpace{}:=\ESHSpace{}l\ESHSpace{}|\}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{204A87}{else}\ESHSpace{}\textcolor[HTML]{346604}{fail})

==> listings/sensor5def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}length\ESHSpace{}(msg.(data))\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}.

==> listings/sensor5enc.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{encode}\ESHSpace{}:=\ESHSpace{}encoder\_impl\ESHSpace{}enc\_dec.\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}stationID\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}data\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}Datatypes.length\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}natToWord\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00000111\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}const\ESHSpace{}0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}11100010\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}data\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}AlignedEncodeList\ESHSpace{}(\textcolor[HTML]{204A87}{\ESHUnicodeSubstitution{\ESHMathSymbol{\lambda}}}\ESHSpace{}\textcolor[HTML]{B35000}{\_}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}high\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte}\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\gg}}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}low\_bits\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ggg}}\ESHSpace{}\textcolor[HTML]{75507B}{SetCurrentByte})

==> listings/sensor6def.v.esh.tex <==
\ESHBol{}\textcolor[HTML]{346604}{Inductive}\ESHSpace{}\textcolor[HTML]{A40000}{reading}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}Temperature\ESHSpace{}(\textcolor[HTML]{B35000}{\_}\ESHSpace{}:\ESHSpace{}word\ESHSpace{}14)\ESHSpace{}|\ESHSpace{}Humidity\ESHSpace{}(\textcolor[HTML]{B35000}{\_}\ESHSpace{}:\ESHSpace{}word\ESHSpace{}14).\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{fmt\_reading}\ESHSpace{}m\ESHSpace{}s\ESHSpace{}:=\ESHSpace{}\textcolor[HTML]{204A87}{match}\ESHSpace{}m\ESHSpace{}\textcolor[HTML]{204A87}{with}\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}Temperature\ESHSpace{}t\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(serialize\ESHSpace{}(0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}00\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}t)\ESHSpace{}s)\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}|\ESHSpace{}Humidity\ESHSpace{}h\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\Rightarrow}}\ESHSpace{}\textcolor[HTML]{346604}{ret}\ESHSpace{}(serialize\ESHSpace{}(0\ESHWeightBold{\textcolor[HTML]{204A87}{b}}01\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\cdot}}\ESHSpace{}h)\ESHSpace{}s)\ESHSpace{}\textcolor[HTML]{204A87}{end}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_reading}\ESHSpace{}:=\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ldots}}.\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Lemma}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_readingCorrect}:\ESHSpace{}CorrectEncoder\ESHSpace{}fmt\_reading\ESHSpace{}enc\_reading.\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ldots}}\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{dec\_reading}\ESHSpace{}:=\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ldots}}.\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Lemma}\ESHSpace{}\textcolor[HTML]{A40000}{dec\_readingCorrect}:\ESHSpace{}CorrectDecoder\ESHSpace{}fmt\_reading\ESHSpace{}dec\_reading.\ESHSpace{}\ESHUnicodeSubstitution{\ESHMathSymbol{\ldots}}\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Ltac}\ESHSpace{}\textcolor[HTML]{A40000}{new\_encoder\_rules}\ESHSpace{}::=\ESHSpace{}\textcolor[HTML]{00008B}{apply}\ESHSpace{}enc\_readingCorrect.\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Ltac}\ESHSpace{}\textcolor[HTML]{A40000}{new\_decoder\_rules}\ESHSpace{}::=\ESHSpace{}\textcolor[HTML]{00008B}{apply}\ESHSpace{}dec\_readingCorrect.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Record}\ESHSpace{}\textcolor[HTML]{A40000}{sensor\_msg}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\{\ESHSpace{}stationID:\ESHSpace{}word\ESHSpace{}8;\ESHSpace{}data:\ESHSpace{}list\ESHSpace{}reading\ESHSpace{}\}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{format}\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\ESHSpace{}\textcolor[HTML]{75507B}{format\_word}\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}stationID\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_nat}\ESHSpace{}8\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}length\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}++\ESHSpace{}\textcolor[HTML]{75507B}{format\_list}\ESHSpace{}fmt\_reading\ESHSpace{}\ESHUnicodeSubstitution{\ensuremath{\circ}}\ESHSpace{}data.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{invariant}\ESHSpace{}(\textcolor[HTML]{B35000}{msg}:\ESHSpace{}sensor\_msg)\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}length\ESHSpace{}(msg.(data))\ESHSpace{}{<}\ESHSpace{}2\ESHRaise{0.50}{8}.\ESHEol
\ESHBol{}\ESHEmptyLine{}\ESHEol
\ESHBol{}\textcolor[HTML]{346604}{Let}\ESHSpace{}\textcolor[HTML]{A40000}{enc\_dec}:\ESHSpace{}EncDecPair\ESHSpace{}format\ESHSpace{}invariant\ESHSpace{}:=\ESHEol
\ESHBol{}\ESHSpace{}\ESHSpace{}\ESHWeightBold{\textcolor[HTML]{75507B}{ltac}}:(\textcolor[HTML]{00008B}{derive\_encoder\_decoder\_pair}).

==> src/Common/Tactics/transparent_abstract_tactics.ml.v84 <==
module TRANSPARENT_ABSTRACT =
struct

  (* [tac] : string representing identifier *)
  (* [args] : tactic arguments *)
  (* [ltac_lcall] : Build a tactic expression calling a variable let-bound to a tactic == [F] args *)
  let ltac_lcall tac args =
    Tacexpr.TacArg(Util.dummy_loc,Tacexpr.TacCall(Util.dummy_loc, Glob_term.ArgVar(Util.dummy_loc, Names.id_of_string tac),args))

  (* [ltac_letin] : Build a let tactic expression. let x := e1 in e2 *)
  let ltac_letin (x, e1) e2 =
    Tacexpr.TacLetIn(false,[(Util.dummy_loc,Names.id_of_string x),e1],e2)

  (* [ltac_apply] : Run a tactic by let binding it... *)
  let ltac_apply (f:Tacexpr.glob_tactic_expr) (args:Tacexpr.glob_tactic_arg list) =
    Tacinterp.eval_tactic
      (ltac_letin ("F", Tacexpr.Tacexp f) (ltac_lcall "F" args))

  (* Lift a constructor to an ltac value. *)
  let to_ltac_val c = Tacexpr.TacDynamic(Util.dummy_loc, Pretyping.constr_in c)

  let interpretable_as_section_decl d1 d2 = match d1,d2 with
    | (_,Some _,_), (_,None,_) -> false
    | (_,Some b1,t1), (_,Some b2,t2) -> Term.eq_constr b1 b2 && Term.eq_constr t1 t2
    | (_,None,t1), (_,_,t2) -> Term.eq_constr t1 t2

  (* Build a new definition for [term] with identifier [id] and call *)
  (* the [tacK] tactic with the result. *)
  let transparent_abstract_term id (term : Term.constr) tacK gl =
    let current_sign = Global.named_context()
    and global_sign = Tacmach.pf_hyps gl in
    let sign,secsign =
      List.fold_right
	(fun (id,_,_ as d) (s1,s2) ->
	 if Termops.mem_named_context id current_sign &&
              interpretable_as_section_decl (Sign.lookup_named id current_sign) d
         then (s1,Environ.push_named_context_val d s2)
	 else (Sign.add_named_decl d s1,s2))
	global_sign (Sign.empty_named_context,Environ.empty_named_context_val) in
    let id = Namegen.next_global_ident_away id (Tacmach.pf_ids_of_hyps gl) in
    let concl = Termops.it_mkNamedProd_or_LetIn (Tacmach.pf_type_of gl term) sign in
    let term =
      try Evarutil.flush_and_check_evars (Tacmach.project gl) term
      with Evarutil.Uninstantiated_evar _ ->
	Util.error "\"abstract\" cannot handle existentials." in
    let concl =
      try Evarutil.flush_and_check_evars (Tacmach.project gl) concl
      with Evarutil.Uninstantiated_evar _ ->
	Util.error "\"abstract\" cannot handle existentials." in
    let prf = Proof_global.give_me_the_proof () in
    let constr = { Entries.const_entry_body = term;
                   const_entry_secctx = Proof.get_used_variables prf;
                   const_entry_type = Some concl;
		   const_entry_opaque = false} in
    let cd = Entries.DefinitionEntry constr in
    let lem = Term.mkConst (Declare.declare_constant ~internal:Declare.KernelSilent id (cd,Decl_kinds.IsDefinition Decl_kinds.Definition)) in
    ltac_apply tacK [to_ltac_val lem] gl

  (* Transparently abstract the goal *)
  let transparent_abstract_by_tac id tac gl =
    let current_sign = Global.named_context()
    and global_sign = Tacmach.pf_hyps gl in
    let sign,secsign =
      List.fold_right
	(fun (id,_,_ as d) (s1,s2) ->
	 if Termops.mem_named_context id current_sign &&
              interpretable_as_section_decl (Sign.lookup_named id current_sign) d
         then (s1,Environ.push_named_context_val d s2)
	 else (Sign.add_named_decl d s1,s2))
	global_sign (Sign.empty_named_context,Environ.empty_named_context_val) in
    let id = Namegen.next_global_ident_away id (Tacmach.pf_ids_of_hyps gl) in
    let concl = Termops.it_mkNamedProd_or_LetIn (Tacmach.pf_concl gl) sign in
    let concl =
      try Evarutil.flush_and_check_evars (Tacmach.project gl) concl
      with Evarutil.Uninstantiated_evar _ ->
	Util.error "\"abstract\" cannot handle existentials." in
    let const = Pfedit.build_constant_by_tactic id secsign concl
						(Tacticals.tclCOMPLETE (Tacticals.tclTHEN (Tacticals.tclDO (List.length sign) Tactics.intro) tac)) in
    let cd = Entries.DefinitionEntry const in
    let lem = Term.mkConst (Declare.declare_constant ~internal:Declare.KernelSilent id (cd,Decl_kinds.IsDefinition Decl_kinds.Definition)) in
    Tactics.exact_no_check
      (Term.applist (lem,List.rev (Array.to_list (Sign.instance_from_named_context sign))))
      gl

  let tclABSTRACT2 name_op tac gl =
    let s = match name_op with
      | Some s -> s
      | None   -> Nameops.add_suffix (Pfedit.get_current_proof_name ()) "_term"
    in
    transparent_abstract_by_tac s (ltac_apply tac []) gl

  let tclABSTRACTTERM name_op term tacK gl =
    let s = match name_op with
      | Some s -> s
      | None   -> Nameops.add_suffix (Pfedit.get_current_proof_name ()) "_term"
    in
    transparent_abstract_term s term tacK gl

end


==> src/Common/Tactics/transparent_abstract_tactics.ml.v85 <==
module TRANSPARENT_ABSTRACT =
  struct
    open Environ
    open Context
    open Termops
    open Evarutil
    open Errors
    open Decl_kinds
    open Pfedit
    open Names
    open Nameops
    open Tacticals.New
    open Tacmach.New
    open Proofview.Notations
    open Safe_typing
    open Proof_global
    (* Copied from tactics.ml *)
    let interpretable_as_section_decl evd d1 d2 = match d2,d1 with
      | (_,Some _,_), (_,None,_) -> false
      | (_,Some b1,t1), (_,Some b2,t2) ->
	 Evd.e_eq_constr_univs evd b1 b2 && Evd.e_eq_constr_univs evd t1 t2
      | (_,None,t1), (_,_,t2) -> Evd.e_eq_constr_univs evd t1 t2

    (* Copied from tactics.ml *)
    let new_exact_no_check c =
      Proofview.Refine.refine ~unsafe:true (fun h -> (h, c))

    (* [tac] : string representing identifier *)
    (* [args] : tactic arguments *)
    (* [ltac_lcall] : Build a tactic expression calling a variable let-bound to a tactic == [F] args *)
    let ltac_lcall tac args =
      Tacexpr.TacArg(Loc.dummy_loc,Tacexpr.TacCall(Loc.dummy_loc, Misctypes.ArgVar(Loc.dummy_loc, Names.id_of_string tac),args))

    (* [ltac_letin] : Build a let tactic expression. let x := e1 in e2 *)
    let ltac_letin (x, e1) e2 =
      Tacexpr.TacLetIn(false,[(Loc.dummy_loc,Names.id_of_string x),e1],e2)

    (* [ltac_apply] : Run a tactic by let binding it... *)
    let ltac_apply (f:Tacexpr.glob_tactic_expr) (args:Tacexpr.glob_tactic_arg list) =
      ltac_letin ("F", Tacexpr.Tacexp f) (ltac_lcall "F" args)

    (* Lift a constr to an ltac value. *)
    let to_ltac_val c = Tacexpr.TacDynamic(Loc.dummy_loc, Pretyping.constr_in c)

    (* Build a new definition for [term] with identifier [id] and call *)
    (* the [tacK] tactic with the result, using [lcl] to decide if the *)
    (* definition is local. *)
    let transparent_abstract_term id (term : Term.constr) tacK gk lcl =
      (* Apply to each goal, normalizing evars in each first. *)
      Proofview.Goal.nf_enter begin
	  fun gl ->
	  let current_sign = Global.named_context()
	  and global_sign = Proofview.Goal.hyps gl in
	  let evdref = ref (Proofview.Goal.sigma gl) in
	  (* Identify which hypotheses are local and which are section variables. *)
	  let sign,secsign =
	    List.fold_right
	      (fun (id,_,_ as d) (s1,s2) ->
	       if mem_named_context id current_sign &&
		    interpretable_as_section_decl evdref (lookup_named id current_sign) d
               then (s1,push_named_context_val d s2)
	       else (add_named_decl d s1,s2))
	      global_sign (empty_named_context,empty_named_context_val) in
	  (* Build the identifier for the new term *)
	  let id = Namegen.next_global_ident_away id (pf_ids_of_hyps gl) in
	  (* Construct the type of the term by abstracting over the *)
	  (* local hypotheses and definitions. *)
	  let (_, termType) = Tacmach.New.pf_type_of gl term in
	  let termType = it_mkNamedProd_or_LetIn termType sign in
	  let termType =
	    try flush_and_check_evars !evdref termType
	    with Uninstantiated_evar _ ->
	      error "\"abstract\" cannot handle existentials." in
	  (* *)
	  let term =
	    try flush_and_check_evars !evdref term
	    with Uninstantiated_evar _ ->
	      error "\"abstract\" cannot handle existentials." in
	  let evd, ctx, termType =
	    (* FIXME: should be done only if the tactic succeeds *)
	    let evd, nf = nf_evars_and_universes !evdref in
	    let ctx = Evd.universe_context_set evd in
	    evd, ctx, nf termType
	  in
	  let constr = { Entries.const_entry_body =
			   Future.from_val ((term ,Univ.ContextSet.empty),
					    Safe_typing.empty_private_constants);
			 (* FIXME: what's the right set of section variables *)
			 const_entry_secctx = Proof_global.get_used_variables ();
			 (* bendy: Not sure how these feedback entries are used. None seems safe? *)
			 const_entry_feedback = None;
			 const_entry_type = Some termType;

			 (* bendy: I assume we don't want polymorphic definitions?*)
			 const_entry_polymorphic = false;
			 const_entry_universes = snd (Evd.universe_context evd);

			 const_entry_opaque = false;
			 (* bendy: again, not sure how this is used, false appears *)
			 (* to be the default in the code base.  *)
			 const_entry_inline_code = false } in
	  (* Create a global definition for const *)
	  let cd = Entries.DefinitionEntry constr in
	  let decl = (cd, IsDefinition Definition) in
	  (** bendy: Seems okay for new constant to be local, but may have unintended **)
	  (** consequences if abstracted terms should be accessed outside the proof. **)
	  let cst = Declare.declare_constant ~internal:Declare.InternalTacticRequest ~local:lcl id decl in
	  let df, ctx = Universes.unsafe_constr_of_global (Globnames.ConstRef cst) in
	  (* Get the universe context associated with the evar map [evd] *)
	  let ectx = Evd.evar_universe_context evd in
	  (* Universe Variable stuff? *)
	  let evd = Evd.set_universe_context evd ectx in
	  (* Build a private constant for the new constant *)
	  let eff = private_con_of_con (Global.safe_env ()) cst in
	  (* Add that constant to the private constants *)
	  let effs = add_private eff
				 Entries.(snd (Future.force constr.const_entry_body)) in
	  Proofview.Unsafe.tclEVARS evd <*>
	    Proofview.tclEFFECTS effs <*>
	    Tacinterp.eval_tactic (ltac_apply tacK [to_ltac_val df])
	end

    (* Solve the goal [gk] by tactic [tak] and save the constructed term as *)
    (* a transparent definition with identifier [id], using [lcl] to decide *)
    (* if the definition is local.  *)
    let transparent_abstract_by_tac id tac gk lcl =
      (* Apply to each goal, normalizing evars in each first. *)
      Proofview.Goal.nf_enter begin
	  fun gl ->
	  let current_sign = Global.named_context()
	  and global_sign = Proofview.Goal.hyps gl in
	  let evdref = ref (Proofview.Goal.sigma gl) in
	  (* Identify which hypotheses are local and which are section variables. *)
	  let sign,secsign =
	    List.fold_right
	      (fun (id,_,_ as d) (s1,s2) ->
	       if mem_named_context id current_sign &&
		    interpretable_as_section_decl evdref (lookup_named id current_sign) d
               then (s1,push_named_context_val d s2)
	       else (add_named_decl d s1,s2))
	      global_sign (empty_named_context,empty_named_context_val) in
	  (* Build the identifier for the new term *)
	  let id = Namegen.next_global_ident_away id (pf_ids_of_hyps gl) in
	  (* Construct the type of the term by abstracting over the *)
	  (* local hypotheses and definitions. *)
	  let concl = it_mkNamedProd_or_LetIn (Proofview.Goal.concl gl) sign in
	  (* Make sure there are no uninstantiated evars in the type of the target. *)
	  let concl =
	    try flush_and_check_evars !evdref concl
	    with Uninstantiated_evar _ ->
	      error "\"abstract\" cannot handle existentials." in
	  (* Normalize evars in the goal, for reasons unknown *)
	  let evd, ctx, concl =
	    (* FIXME: should be done only if the tactic succeeds *)
	    let evd, nf = nf_evars_and_universes !evdref in
	    let ctx = Evd.universe_context_set evd in
	    evd, ctx, nf concl
	  in
	  (* This is the tactic script that should solve the goal. *)
	  let solve_tac = tclCOMPLETE (tclTHEN (tclDO (List.length sign) Tactics.intro) tac) in
	  (* Get the universe context associated with the evar map [evd] *)
	  let ectx = Evd.evar_universe_context evd in
	  let (const, safe, ectx) =
	    (* Actually build the constant using [solve_tac] *)
	    try Pfedit.build_constant_by_tactic ~goal_kind:gk id ectx secsign concl solve_tac
	    with Logic_monad.TacticFailure e as src ->
	      (* if the tactic [tac] fails, it reports a [TacticFailure e], *)
	      (* which is an error irrelevant to the proof system (in fact it *)
	      (* means that [e] comes from [tac] failing to yield enough *)
	      (* success). Hence it reraises [e]. *)
	      let (_, info) = Errors.push src in
	      Exninfo.iraise (e, info)
	  in
	  (* Create a global definition for const *)
	  let cd = Entries.DefinitionEntry const in
 	  let decl = (cd, IsDefinition Definition) in
	  (** bendy: Seems okay for new constant to be local, but may have unintended **)
	  (** consequences if abstracted terms should be accessed outside the proof. **)
	  let cst = Declare.declare_constant ~internal:Declare.InternalTacticRequest ~local:lcl id decl in
	  (* Tactic Monad *)
	  let df, ctx = Universes.unsafe_constr_of_global (Globnames.ConstRef cst) in
	  (* Universe Variable stuff? *)
	  let evd = Evd.set_universe_context evd ectx in
	  (* Build a private constant for the new constant *)
	  let eff = private_con_of_con (Global.safe_env ()) cst in
	  (* Add that constant to the private constants *)
	  let effs = add_private eff
				 Entries.(snd (Future.force const.const_entry_body)) in
	  (* Get the local arguments to apply the new constant to. *)
	  let args = List.rev (instance_from_named_context sign) in
	  (* Use the definition built above to solve the goal. *)
	  let solve =
	    Proofview.Unsafe.tclEVARS evd <*>
	      Proofview.tclEFFECTS effs <*>
	      new_exact_no_check (Term.applist (df, args))
	  in
	  if not safe then Proofview.mark_as_unsafe <*> solve else solve
	end

    (* Default identifier *)
    let anon_id = Id.of_string "anonymous"

    let tclTRABSTRACT name_op tac =
      (* What's the right default goal kind?*)
      let default_gk = (Global, false, Proof Theorem) in
      let s, gk = match name_op with
	| Some s ->
	   (try let _, gk, _ = current_proof_statement () in s, gk
	    with NoCurrentProof -> s, default_gk)
	| None   ->
	   let name, gk =
	     try let name, gk, _ = current_proof_statement () in name, gk
	     with NoCurrentProof -> anon_id, default_gk in
	   add_suffix name "_term", gk
      in
      transparent_abstract_by_tac s tac gk false

    let tclABSTRACTTERM name_op term tacK =
      (* What's the right default goal kind?*)
      let default_gk = (Global, false, Proof Theorem) in
      let s, gk = match name_op with
	| Some s ->
	   (try let _, gk, _ = current_proof_statement () in s, gk
	    with NoCurrentProof -> s, default_gk)
	| None   ->
	   let name, gk =
	     try let name, gk, _ = current_proof_statement () in name, gk
	     with NoCurrentProof -> anon_id, default_gk in
	   add_suffix name "_term", gk
      in
      transparent_abstract_term s term tacK gk false
  end

    (*let tclABSTRACT2 name_op tac gl =
    let s = match name_op with
      | Some s -> s
      | None   -> Nameops.add_suffix (Pfedit.get_current_proof_name ()) "_term"
    in *)


==> src/Common/Tactics/transparent_abstract_tactics.ml.v86 <==
module TRANSPARENT_ABSTRACT =
  struct
    open Environ
    open Context
    open Termops
    open Evarutil
    open CErrors
    open Decl_kinds
    open Pfedit
    open Names
    open Nameops
    open Tacticals.New
    open Tacmach.New
    open Proofview.Notations
    open Safe_typing
    open Proof_global
    open Sigma.Notations
    (* Copied from tactics.ml *)
    let interpretable_as_section_decl evd d1 d2 =
      let open Context.Named.Declaration in
      match d2, d1 with
      | LocalDef _, LocalAssum _ -> false
      | LocalDef (_,b1,t1), LocalDef (_,b2,t2) ->
        Evd.e_eq_constr_univs evd b1 b2 && Evd.e_eq_constr_univs evd t1 t2
      | LocalAssum (_,t1), d2 -> Evd.e_eq_constr_univs evd t1 (get_type d2)

    (* [tac] : string representing identifier *)
    (* [args] : tactic arguments *)
    (* [ltac_lcall] : Build a tactic expression calling a variable let-bound to a tactic == [F] args *)
    let ltac_lcall tac args =
      Tacexpr.TacArg(Loc.dummy_loc,Tacexpr.TacCall(Loc.dummy_loc, Misctypes.ArgVar(Loc.dummy_loc, Names.id_of_string tac),args))

    (* [ltac_letin] : Build a let tactic expression. let x := e1 in e2 *)
    let ltac_letin (x, e1) e2 =
      Tacexpr.TacLetIn(false,[(Loc.dummy_loc,Names.id_of_string x),e1],e2)

    (* [ltac_apply] : Run a tactic with arguments... *)
    let ltac_apply (f: Tacinterp.Value.t) (arg:Tacinterp.Value.t) =
      let open Geninterp in
      let ist = Tacinterp.default_ist () in
      let id = Id.of_string "X" in
      let idf = Id.of_string "F" in
      let ist = { ist with Tacinterp.lfun = Id.Map.add idf f (Id.Map.add id arg ist.lfun) } in
      let arg = Tacexpr.Reference (Misctypes.ArgVar (Loc.ghost, id)) in
      Tacinterp.eval_tactic_ist ist
        (ltac_lcall "F" [arg])

    (* Lift a constr to an ltac value. *)
    let to_ltac_val c = Tacinterp.Value.of_constr c

    (* Build a new definition for [term] with identifier [id] and call *)
    (* the [tacK] tactic with the result, using [lcl] to decide if the *)
    (* definition is local. *)
    let transparent_abstract_term id (term : Term.constr) tacK gk lcl =
      let open Tacticals.New in
      let open Tacmach.New in
      let open Proofview.Notations in
      let open Context.Named.Declaration in
      (* Apply to each goal, normalizing evars in each first. *)
      Proofview.Goal.nf_enter { enter = begin
                fun gl ->
          let sigma = Proofview.Goal.sigma gl in
          let current_sign = Global.named_context_val()
          and global_sign = Proofview.Goal.hyps gl in
          let sigma = Sigma.to_evar_map sigma in
          let evdref = ref sigma in
          (* Identify which hypotheses are local and which are section variables. *)
          let sign,secsign =
            List.fold_right
              (fun d (s1,s2) ->
               let id = get_id d in
               if mem_named_context_val id current_sign &&
                    interpretable_as_section_decl evdref (lookup_named_val id current_sign) d
               then (s1,push_named_context_val d s2)
               else (Context.Named.add d s1,s2))
              global_sign (Context.Named.empty,empty_named_context_val) in
          (* Build the identifier for the new term *)
          let id = Namegen.next_global_ident_away id (pf_ids_of_hyps gl) in
          (* Construct the type of the term by abstracting over the *)
          (* local hypotheses and definitions. *)
          let (_, termType) = Tacmach.New.pf_type_of gl term in
          let termType = it_mkNamedProd_or_LetIn termType sign in
          let termType =
            try flush_and_check_evars !evdref termType
            with Uninstantiated_evar _ ->
              error "\"abstract\" cannot handle existentials." in
          (* *)
          let term =
            try flush_and_check_evars !evdref term
            with Uninstantiated_evar _ ->
              error "\"abstract\" cannot handle existentials." in
          let evd, ctx, termType =
            (* FIXME: should be done only if the tactic succeeds *)
            let evd, nf = nf_evars_and_universes !evdref in
            let ctx = Evd.universe_context_set evd in
            evd, ctx, nf termType
          in
          let constr = { Entries.const_entry_body =
                           Future.from_val ((term ,Univ.ContextSet.empty),
                                            Safe_typing.empty_private_constants);
                         (* FIXME: what's the right set of section variables *)
                         const_entry_secctx = Proof_global.get_used_variables ();
                         (* bendy: Not sure how these feedback entries are used. None seems safe? *)
                         const_entry_feedback = None;
                         const_entry_type = Some termType;

                         (* bendy: I assume we don't want polymorphic definitions?*)
                         const_entry_polymorphic = false;
                         const_entry_universes = snd (Evd.universe_context evd);

                         const_entry_opaque = false;
                         (* bendy: again, not sure how this is used, false appears *)
                         (* to be the default in the code base.  *)
                         const_entry_inline_code = false } in
          (* Create a global definition for const *)
          let cd = Entries.DefinitionEntry constr in
          let decl = (cd, IsDefinition Definition) in
          (** bendy: Seems okay for new constant to be local, but may have unintended **)
          (** consequences if abstracted terms should be accessed outside the proof. **)
          let cst = Declare.declare_constant ~internal:Declare.InternalTacticRequest ~local:lcl id decl in
          let df, ctx = Universes.unsafe_constr_of_global (Globnames.ConstRef cst) in
          (* Get the universe context associated with the evar map [evd] *)
          let ectx = Evd.evar_universe_context evd in
          (* Universe Variable stuff? *)
          let evd = Evd.set_universe_context evd ectx in
          (* Build a private constant for the new constant *)
          let eff = private_con_of_con (Global.safe_env ()) cst in
          (* Add that constant to the private constants *)
          let effs = add_private eff
                                 Entries.(snd (Future.force constr.const_entry_body)) in
          Proofview.Unsafe.tclEVARS evd <*>
            Proofview.tclEFFECTS effs <*>
            ltac_apply tacK (Tacinterp.Value.of_constr df)
        end }

    (* Solve the goal [gk] by tactic [tak] and save the constructed term as *)
    (* a transparent definition with identifier [id], using [lcl] to decide *)
    (* if the definition is local.  *)
    let transparent_abstract_by_tac id tac gk lcl =
      let open Tacticals.New in
      let open Tacmach.New in
      let open Proofview.Notations in
      let open Context.Named.Declaration in
      (* Apply to each goal, normalizing evars in each first. *)
      Proofview.Goal.nf_enter { enter = begin
          fun gl ->
          let sigma = Proofview.Goal.sigma gl in
          let current_sign = Global.named_context_val()
          and global_sign = Proofview.Goal.hyps gl in
          let sigma = Sigma.to_evar_map sigma in
          let evdref = ref sigma in
          (* Identify which hypotheses are local and which are section variables. *)
          let sign,secsign =
            List.fold_right
              (fun d (s1,s2) ->
               let id = get_id d in
               if mem_named_context_val id current_sign &&
                    interpretable_as_section_decl evdref (lookup_named_val id current_sign) d
               then (s1,push_named_context_val d s2)
               else (Context.Named.add d s1,s2))
              global_sign (Context.Named.empty,empty_named_context_val) in
          (* Build the identifier for the new term *)
          let id = Namegen.next_global_ident_away id (pf_ids_of_hyps gl) in
          (* Construct the type of the term by abstracting over the *)
          (* local hypotheses and definitions. *)
          let concl = it_mkNamedProd_or_LetIn (Proofview.Goal.concl gl) sign in
          (* Make sure there are no uninstantiated evars in the type of the target. *)
          let concl =
            try flush_and_check_evars !evdref concl
            with Uninstantiated_evar _ ->
              error "\"abstract\" cannot handle existentials." in
          (* Normalize evars in the goal, for reasons unknown *)
          let evd, ctx, concl =
            (* FIXME: should be done only if the tactic succeeds *)
            let evd, nf = nf_evars_and_universes !evdref in
            let ctx = Evd.universe_context_set evd in
            evd, ctx, nf concl
          in
          (* This is the tactic script that should solve the goal. *)
          let solve_tac = tclCOMPLETE (tclTHEN (tclDO (List.length sign) Tactics.intro) tac) in
          (* Get the universe context associated with the evar map [evd] *)
          let ectx = Evd.evar_universe_context evd in
          let (const, safe, ectx) =
            (* Actually build the constant using [solve_tac] *)
            try Pfedit.build_constant_by_tactic ~goal_kind:gk id ectx secsign concl solve_tac
            with Logic_monad.TacticFailure e as src ->
              (* if the tactic [tac] fails, it reports a [TacticFailure e], *)
              (* which is an error irrelevant to the proof system (in fact it *)
              (* means that [e] comes from [tac] failing to yield enough *)
              (* success). Hence it reraises [e]. *)
              let (_, info) = CErrors.push src in
              Exninfo.iraise (e, info)
          in
          (* Create a global definition for const *)
          let cd = Entries.DefinitionEntry const in
           let decl = (cd, IsDefinition Definition) in
          (** bendy: Seems okay for new constant to be local, but may have unintended **)
          (** consequences if abstracted terms should be accessed outside the proof. **)
          let cst = Declare.declare_constant ~internal:Declare.InternalTacticRequest ~local:lcl id decl in
          (* Tactic Monad *)
          let df, ctx = Universes.unsafe_constr_of_global (Globnames.ConstRef cst) in
          (* Universe Variable stuff? *)
          let evd = Evd.set_universe_context evd ectx in
          (* Build a private constant for the new constant *)
          let eff = private_con_of_con (Global.safe_env ()) cst in
          (* Add that constant to the private constants *)
          let effs = add_private eff
                                 Entries.(snd (Future.force const.const_entry_body)) in
          (* Get the local arguments to apply the new constant to. *)
          let args = List.rev (Context.Named.to_instance sign) in
          (* Use the definition built above to solve the goal. *)
          let solve =
            Proofview.Unsafe.tclEVARS evd <*>
              Proofview.tclEFFECTS effs <*>
              Tactics.exact_no_check (Term.applist (df, args))
          in
          if not safe then Proofview.mark_as_unsafe <*> solve else solve
        end }

    (* Default identifier *)
    let anon_id = Id.of_string "anonymous"

    let tclTRABSTRACT name_op tac =
      (* What's the right default goal kind?*)
      let default_gk = (Global, false, Proof Theorem) in
      let s, gk = match name_op with
        | Some s ->
           (try let _, gk, _ = current_proof_statement () in s, gk
            with NoCurrentProof -> s, default_gk)
        | None   ->
           let name, gk =
             try let name, gk, _ = current_proof_statement () in name, gk
             with NoCurrentProof -> anon_id, default_gk in
           add_suffix name "_term", gk
      in
      transparent_abstract_by_tac s tac gk false

    let tclABSTRACTTERM name_op term tacK =
      (* What's the right default goal kind?*)
      let default_gk = (Global, false, Proof Theorem) in
      let s, gk = match name_op with
        | Some s ->
           (try let _, gk, _ = current_proof_statement () in s, gk
            with NoCurrentProof -> s, default_gk)
        | None   ->
           let name, gk =
             try let name, gk, _ = current_proof_statement () in name, gk
             with NoCurrentProof -> anon_id, default_gk in
           add_suffix name "_term", gk
      in
      transparent_abstract_term s term tacK gk false
  end

    (*let tclABSTRACT2 name_op tac gl =
    let s = match name_op with
      | Some s -> s
      | None   -> Nameops.add_suffix (Pfedit.get_current_proof_name ()) "_term"
    in *)

